Quantum holography with undetected light

Holography exploits the interference of light fields to obtain a systematic reconstruction of the light fields wavefronts. Classical holography techniques have been very successful in diverse areas such as microscopy, manufacturing technology, and basic science. Extending holographic methods to the level of single photons has been proven challenging, since applying classical holography techniques to this regime pose technical problems. Recently the retrieval of the spatial structure of a single photon, using another photon under experimental control with a well-characterized spatial shape as reference, was demonstrated using the intrinsically non-classical Hong-Ou-Mandel interference on a beam splitter. Here we present a method for recording a hologram of single photons without detecting the photons themselves, and importantly, with no need to use a well-characterized companion reference photon. Our approach is based on quantum interference between two-photon probability amplitudes in a nonlinear interferometer. As in classical holography, the hologram of a single photon allows retrieving the complete information about the "shape" of the photon (amplitude and phase) despite the fact that the photon is never detected.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
